Learning Retrieval Models with Sparse Autoencoders

Sparse autoencoders (SAEs) provide a powerful mechanism for decomposing the dense representations produced by Large Language Models (LLMs) into interpretable latent features. We posit that SAEs constitute a natural foundation for Learned Sparse Retrieval (LSR), whose objective is to encode queries and documents into high-dimensional sparse representations optimized for efficient retrieval. In contrast to existing LSR approaches that project input sequences into the vocabulary space, SAE-based representations offer the potential to produce more semantically structured, expressive, and language-agnostic features. Building on this insight, we introduce SPLARE, a method to train SAE-based LSR models. Our experiments, relying on recently released open-source SAEs, demonstrate that this technique consistently outperforms vocabulary-based LSR in multilingual and out-of-domain settings. SPLARE-7B, a multilingual retrieval model capable of producing generalizable sparse latent embeddings for a wide range of languages and domains, achieves top results on MMTEB's multilingual and English retrieval tasks. We also developed a 2B-parameter variant with a significantly lighter footprint.

==> interpretability_examples/code_4.tex <==
\begin{retrievalexample}{from CodeEditSearchRetrieval}
\sffamily\small
\footnotesize
\textbf{Query}: \textsf{Use more predictable demo IP address
}\\
\textbf{Positive document}: \textsf{--- 
+++ 
@@ -6,7 +6,7 @@
 def main():
     session = sessions.Session(
         target=sessions.Target(
-            connection=SocketConnection("192.168.56.101", 8021, proto='tcp')))
+            connection=SocketConnection("127.0.0.1", 8021, proto='tcp')))
 
     s\_initialize("user")
     s\_string("USER")}\\[3pt]
\normalsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l r | l r@{}}
\toprule
\multicolumn{2}{c}{\textbf{SPLARE — top features} (document rank = 25)} & \multicolumn{2}{c}{\textbf{SPLADE — top tokens} (document rank = 3)} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-4}
Explanation (from Neuronpedia \cite{neuronpedia}) & \% & Token & \% \\
\midrule
technical terms and configurations related to networking and server connections &  20.2 & \texttt{\textvisiblespace localhost} &   8.5 \\
 elements related to network connection and configuration &  15.8 & \texttt{\textvisiblespace address} &   7.0 \\
 references to local server configurations and network connections &  14.6 & \texttt{\textvisiblespace ip} &   6.4 \\
 terminology and concepts related to VPN protocols and security vulnerabilities &  12.2 & \texttt{\textvisiblespace IP} &   6.2 \\
 programming-related terms and functions &   6.3 & \texttt{\textvisiblespace test} &   3.9 \\
 instances of web-related technical configurations and programming tasks &   5.6 & \texttt{\textvisiblespace local} &   3.9 \\
 financial terms and documents related to transactions &   5.5 & \texttt{\textvisiblespace server} &   3.6 \\
 references to product demonstrations and testing &   4.1 & \texttt{127} &   3.4 \\
technical terms related to internet security and protocols &   3.6 & \texttt{\textvisiblespace virtual} &   3.2 \\
 references to institutions or organizations in a structured context &   3.5 & \texttt{address} &   3.0 \\
\bottomrule
\end{tabular}}
\label{ref:example_code_4}
\end{retrievalexample}

==> interpretability_examples/splare_good_splade_bad.tex <==
\begin{retrievalexample}{Retrieval example from MSMarco test \cite{bajaj2018msmarcohumangenerated}}
\label{example:main}
\sffamily\small
\footnotesize
\textbf{Query}:\textsf{which health care system provides all citizens or residents with equal access to health care services}\\
\textbf{Positive document}: \textsf{Universal Health Care which is also known as universal care, universal coverage or universal health coverage is a term that is used to address a health care system which provides health care and financial protection to every citizen of a specific country.}\\[3pt]
\normalsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l r | l r@{}}
\toprule
\multicolumn{2}{c}{\textbf{SPLARE} (doc rank = 3)} & \multicolumn{2}{c}{\textbf{SPLADE} (doc rank = 20)} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-4}
Top scoring features & \% & Top scoring tokens & \% \\
\midrule
 concepts related to healthcare systems and government involvement &   9.8 & \texttt{\textvisiblespace universal} &   7.4 \\
mentions of "system" and its variations in various contexts &   5.5 & \texttt{\textvisiblespace healthcare} &   7.0 \\
terminology related to citizenship and citizens' rights &   5.0 & \texttt{\textvisiblespace care} &   5.9 \\
 terms related to healthcare and medical professions &   4.9 & \texttt{\textvisiblespace health} &   5.5 \\
terms related to access and equity in education and essential services &   4.7 & \texttt{\textvisiblespace system} &   5.5 \\
references to health-related technology and community health initiatives &   4.1 & \texttt{\textvisiblespace Universal} &   5.3 \\
terms associated with health and well-being &   3.9 & \texttt{\textvisiblespace coverage} &   4.1 \\
 mentions of the criminal justice system and its related issues &   3.6 & \texttt{\textvisiblespace Health} &   3.8 \\
 references to people and their roles in healthcare discussions &   3.4 & \texttt{\textvisiblespace Healthcare} &   3.6 \\
 key terms related to health care quality and individualized patient care &   3.3 & \texttt{\textvisiblespace UNIVERS} &   3.3 \\
\bottomrule
\end{tabular}}
\label{ref:splare_good_splade_bad}
\end{retrievalexample}

==> tables/avg_results_splare.tex <==
\begin{figure}[ht]
    \centering
    \small
    % Left table
    \begin{minipage}{0.48\textwidth}
        \centering
        \captionof{table}{{\it (Left)} Comparison of SPLARE and SPLADE on various MTEB retrieval splits.}
        \begin{tabular}{lcc}
    \toprule
    & SPLADE-Llama & SPLARE \\
    \midrule
    Eng & 58.4 & 58.6 \\ 
    Multilingual & 60.3 & 60.9 \\
    Code & 63.6 & 60.7 \\
    Medical & 67.1 & 68.0 \\
    Law & 57.5 & 58.1  \\
    ChemTEB & 75.7 & 77.2 \\
    BRIGHT & 18.8 & 19.3 \\
    \bottomrule
    \end{tabular}
    \label{table:avg_left}
    \end{minipage}\hfill
    % Right table
    \begin{minipage}{0.48\textwidth}
        \centering
        \captionof{table}{{\it (Right)} Multilingual comparison of SPLARE and SPLADE, including MIRACL and XTREME-UP.}
        \begin{tabular}{lcc}
    \toprule
   & SPLADE-Llama & SPLARE \\
   \midrule
    indic & 90.1 & 91.2 \\
    sca & 70.4 & 70.4 \\
    deu & 55.4 &  56.2 \\
    fra &  65.6 &  65.6 \\
    jpn & &  \\
    kor & 73.7 & 74.9 \\
    rus &  &  \\
    \midrule
    MIRACL & - \\
    XTREME-UP & 56.3 & 59.8 \\
    \bottomrule
    \end{tabular}
    \label{table:avg_right}
    \end{minipage}
\end{figure}

==> tables/full_results/english_all_avg.tex <==
\begin{table}[t]
\caption{Performance of ensligh-data Splare and competitors, on MTEB splits.}
\label{tab:english_results}
\centering
    \begin{tabular}{lcccccc}
    \toprule
    &  Eng & Multilingual & Code & Medical & Law &\textbf{Avg.} \\
    \midrule
    SPLADE-v3  &  50.7 & 38.1 & 44.5 & 44.2 & 40.4 & 43.6 \\
    Lion-SP-8B    & 48.5 & 50.0 & 53.3 & 54.4 & 48.5 & 50.9 \\
    SPLADE-Llama  &  \textbf{52.9} & 54.3 & \textbf{57.3} & 61.0 & 49.0 & 54.9 \\
    SPLARE   &  \textbf{52.9} & \textbf{56.3} & 55.1 & \textbf{62.9} & \textbf{51.2} & \textbf{55.7} \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/full_results/mteb_chem.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\textbf{Task Name} & \textbf{L26\_v0} & \textbf{L26\_v1} & \textbf{l22} & \textbf{llama-splade\_v0} \\
ChemHotpotQARetrieval & 87.9 & 89.3 & 84.8 & 82.1 \\
ChemNQRetrieval & 73.0 & 65.1 & 68.6 & 69.2 \\
\textbf{Average} & \textbf{80.4} & \textbf{77.2} & \textbf{76.7} & \textbf{75.7} \\
\end{tabular}
\caption{Table of task performance across different models.}
\label{table:mteb_chem}
\end{table}

==> tables/full_results/mteb_code.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\textbf{Task Name} & \textbf{L26\_v0} & \textbf{L26\_v1} & \textbf{l22} & \textbf{llama-splade\_v0} \\
AppsRetrieval & 28.8 & 22.6 & 22.6 & 29.5 \\
COIRCodeSearchNetRetrieval & 62.3 & 61.0 & 62.7 & 72.7 \\
CodeEditSearchRetrieval & 74.1 & 72.9 & 73.5 & 74.4 \\
CodeFeedbackMT & 51.1 & 50.3 & 49.5 & 49.4 \\
CodeFeedbackST & 77.5 & 76.3 & 75.7 & 77.9 \\
CodeSearchNetCCRetrieval & 64.3 & 60.4 & 59.0 & 65.1 \\
CodeSearchNetRetrieval & 85.2 & 83.4 & 83.2 & 86.5 \\
CodeTransOceanContest & 84.6 & 81.6 & 85.7 & 86.6 \\
CodeTransOceanDL & 35.1 & 36.3 & 35.1 & 32.0 \\
CosQA & 31.9 & 30.2 & 27.7 & 30.9 \\
StackOverflowQA & 88.9 & 86.0 & 86.9 & 90.2 \\
SyntheticText2SQL & 68.3 & 67.5 & 65.9 & 67.9 \\
\textbf{Average} & \textbf{62.7} & \textbf{60.7} & \textbf{60.6} & \textbf{63.6} \\
\end{tabular}
\caption{Code.}
\label{table:mteb_code}
\end{table}

==> tables/full_results/mteb_law.tex <==
\begin{table}[h]
\label{table:mteb_law}
\centering
\begin{tabular}{lcccc}
\textbf{Task Name} & \textbf{L26\_v0} & \textbf{L26\_v1} & \textbf{l22} & \textbf{llama-splade\_v0} \\
AILACasedocs & 34.5 & 36.2 & 33.4 & 36.5 \\
AILAStatutes & 37.5 & 33.8 & 37.5 & 34.1 \\
GerDaLIRSmall & 28.5 & 27.5 & 26.9 & 27.6 \\
LeCaRDv2 & 61.3 & 62.1 & 60.1 & 58.6 \\
LegalBenchConsumerContractsQA & 84.1 & 86.9 & 86.1 & 84.6 \\
LegalBenchCorporateLobbying & 91.3 & 95.3 & 95.9 & 95.1 \\
LegalQuAD & 55.1 & 55.4 & 55.3 & 55.2 \\
LegalSummarization & 65.7 & 67.8 & 66.7 & 68.4 \\
\textbf{Average} & \textbf{57.2} & \textbf{58.1} & \textbf{57.7} & \textbf{57.5} \\
\end{tabular}
\caption{Table of task performance across different models}
\end{table}

==> tables/full_results/mteb_medical.tex <==
\begin{table}[h]
\label{table:medical}
\centering
\begin{tabular}{lcccc}
\textbf{Task Name} & \textbf{L26\_v0} & \textbf{L26\_v1} & \textbf{l22} & \textbf{llama-splade\_v0} \\
CUREv1 & 56.8 & 63.7 & 59.2 & 56.3 \\
CmedqaRetrieval & 31.1 & 28.0 & 31.8 & 32.2 \\
MedicalQARetrieval & 73.1 & 74.8 & 74.0 & 75.2 \\
NFCorpus & 38.5 & 40.0 & 39.4 & 38.7 \\
PublicHealthQA & 85.2 & 85.7 & 85.3 & 86.0 \\
SciFact & 78.0 & 77.8 & 77.1 & 77.1 \\
SciFact-PL & 74.8 & 75.6 & 73.2 & 73.7 \\
TRECCOVID & 77.1 & 83.4 & 85.7 & 81.1 \\
TRECCOVID-PL & 80.7 & 82.8 & 82.8 & 83.5 \\
\textbf{Average} & \textbf{66.1} & \textbf{68.0} & \textbf{67.6} & \textbf{67.1} \\
\end{tabular}
\caption{Table of task performance across different models}
\end{table}

==> tables/multi-lingual-comp1.tex <==
\begin{table}[t]
\caption{TODO}
\label{tab:multi-lingual-comp:domain}
\centering
    \begin{tabular}{lcc}
    \toprule
    & SPLADE & SPLARE \\
    \midrule
    Eng & 58.4 & 58.6 \\ 
    Multilingual & 60.3 & 60.9 \\
    Code & 63.6 & 60.7 \\
    Medical & 67.1 & 68.0 \\
    Law & 57.5 & 58.1  \\
    ChemTEB & 75.7 & 77.2 \\
    BRIGHT & 18.8 & 19.3 \\
    \bottomrule
    \end{tabular}
\end{table}

